Simulating the dynamics of time-dependent Hamiltonians with a truncated Dyson series

We provide a general method for efficiently simulating time-dependent Hamiltonian dynamics on a circuit-model based quantum computer. Our approach is based on approximating the truncated Dyson series of the evolution operator, extending the earlier proposal by Berry to evolution generated by explicitly time-dependent Hamiltonians. Two alternative strategies are proposed to implement time ordering while exploiting the superposition principle for sampling the Hamiltonian at different times. The resource cost of our simulation algorithm retains the optimal logarithmic dependence on the inverse of the desired precision.

==> W.tex <==
\begin{tiny}
$$
\Qcircuit @C=0.3em @R=0.3em { 
\lstick{k_1}           &\qw&\multigate{6}{\begin{minipage}{3.2em}\!\! prepare\newline \ \ clock\end{minipage}\!} 
&\ctrl{4}&\qw&\dots&&\qw&\qw&\dots&&\qw&\qw                       &\qw &\dots &           &\qw &\qw &\dots &     &\qw &\qw  &\qw       &\dots &       &\qw &\qw  &\qw       &\dots &   &\qw &\ctrl{4}  &\multigate{6}{\begin{minipage}{3.2em}\!\! prepare\newline \ \ clock$^{\dagger}$\end{minipage}\!}   &\qw\\
\lstick{k_k}           &\qw&\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}
&\qw&\qw&\dots&&\ctrl{4}&\qw&\dots&&\qw&\qw                       &\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\qw  &\qw       &\dots &        &\qw &\ctrl{4}  &\qw       &\dots &  &\qw  & \qw&\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}    &\qw \\
\lstick{k_K}           &\qw&\ghost{\begin{minipage}{3.2em}prepare\newline clock\end{minipage}\!}
&\qw&\qw&\dots&&\qw&\qw& \dots&&\ctrl{4}&\qw                      &\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\ctrl{4}    &\qw    &\dots &  &\qw &\qw  &\qw       &\dots &&\qw   &\qw&\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}     &\qw              \\
\lstick{t_1}           &{/}\qw&\ghost{\begin{minipage}{3.2em} prepare\newline  clock \end{minipage}\!}
&\ctrl{4}&\qw&\dots&&\qw&\qw&\dots&&\qw&\qw                       &\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\qw   &\qw       &\dots &   &\qw &\qw  &\qw       &\dots &  &\qw  &\ctrl{4}  &\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}     &\qw\\
\lstick{t_k}           &{/}\qw&\ghost{\begin{minipage}{3.2em} prepare\newline  clock \end{minipage}\!}
&\qw&\qw&\dots&&\ctrl{4}&\qw& \dots&&\qw&\qw                      &\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\qw    &\qw    &\dots &  &\qw &\ctrl{4}  &\qw       &\dots & &\qw  &\qw  &\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}   &\qw \\
\lstick{t_K}           &{/}\qw&\ghost{\begin{minipage}{3.2em} prepare\newline  clock \end{minipage}\!}
&\qw&\qw&\dots&&\qw&\qw&\dots&&\ctrl{4}&\qw                       &\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\ctrl{4}    &\qw    &\dots  &  &\qw  &\qw    &\qw    &\dots & &\qw  &\qw  &\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}    &\qw \\
\lstick{\ket{0\dots 0}}&{/}\qw&\ghost{\begin{minipage}{3.2em} prepare\newline  clock \end{minipage}\!}
&\qw&\qw&\dots&&\qw&\qw&\dots&&\qw&\qw                            &\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\qw    &\qw    &\dots &   &\qw  &\qw    &\qw    &\dots & &\qw  &\qw  &\ghost{\begin{minipage}{3.2em}\!prepare\newline clock\end{minipage}\!}    &\qw\\
\lstick{l_1}           &{/}\qw&\qw  
&\multigate{0}{\alpha(t)}&\qw&\dots&&\qw&\qw&\dots&               &\qw&\ctrl{3}&\qw &\dots &           &\qw &\qw &\dots &     &\qw  &\qw   &\qw       &\dots &     &\qw  &\qw    &\qw    &\dots &  &\qw  &\multigate{0}{\alpha(t)}  &\qw        &\qw\\
\lstick{l_k}           &{/}\qw&\qw   
&\qw&\qw&\dots&&\multigate{0}{\alpha(t)}                          &\qw&\dots&             &\qw&\qw      &\qw &\dots &           &\ctrl{2} &\qw &\dots &     &\qw  &\qw    &\qw     &\dots & &\qw  &\multigate{0}{\alpha^{\dagger}(t)}     &\qw    &\dots & &\qw  &\qw  &\qw    & \qw \\
\lstick{l_K}           &{/}\qw&\qw    
&\qw&\qw&\dots&&\qw&\qw&\dots&&\multigate{0}{\alpha(t)}&\qw       &\qw &\dots &           &\qw &\qw &\dots &     &\ctrl{1}      
&\multigate{0}{\alpha^{\dagger}(t)}  &\qw &\dots  &     &\qw   &\qw  &\qw    &\qw    &\dots &  &\qw  &\qw  &\qw       \\
\lstick{\ket{data}}    &{/}\qw&\qw   
&\qw&\qw&\dots&&\qw&\qw&\dots&&\qw                                &\multigate{0}{-iH_{l_1} }&\qw &\dots & &\multigate{0}{-iH_{l_k} }&\qw  &\dots &   &\multigate{0}{-iH_{l_K} }   &\qw 
&\qw &\dots &  &\qw  &\qw    &\qw    &\dots &    &\qw      &\qw      &\qw  &\qw  
}
$$
\end{tiny}
